A Theoretical and Computational Analysis of Full Strong-Branching

Full strong-branching is a well-known variable selection rule that is known experimentally to produce significantly smaller branch-and-bound trees in comparison to all other known variable selection rules. In this paper, we attempt an analysis of the performance of the strong-branching rule both from a theoretical and a computational perspective. On the positive side for strong-branching we identify vertex cover as a class of instances where this rule provably works well. In particular, for vertex cover we present an upper bound on the size of the branch-and-bound tree using strong-branching as a function of the additive integrality gap, show how the Nemhauser-Trotter property of persistency which can be used as a pre-solve technique for vertex cover is being recursively and consistently used throughout the strong-branching based branch-and-bound tree, and finally provide an example of a vertex cover instance where not using strong-branching leads to a tree that has at least exponentially more nodes than the branch-and-bound tree based on strong-branching. On the negative side for strong-branching, we identify another class of instances where strong-branching based branch-and-bound tree has exponentially larger tree in comparison to another branch-and-bound tree for solving these instances. On the computational side, we conduct experiments on various types of instances to understand how much larger is the size of the strong-branching based branch-and-bound tree in comparison to the optimal branch-and-bound tree. The main take-away from these experiments is that for all these instances, the size of the strong-branching based branch-and-bound tree is within a factor of two of the size of the optimal branch-and-bound tree.

==> tables/table_gen_cropcube1.tex <==
\begin{table}\small
\begin{center}
\caption{Computational Results for Generalized Cropped Cube, $n = 9$}
\begin{adjustwidth}{-1in}{-0.5in}
\begin{tabular}{crrrrrrrrrcrrrrrrr}
\cline{1-8} \cline{11-18}
\multicolumn{1}{c}{\textbf{Index}} & \textbf{q} & \textbf{p} & \multicolumn{1}{p{1cm}}{\textbf{Opt Tree}} & \multicolumn{1}{p{1cm}}{\textbf{SB-L}} & \multicolumn{1}{p{1cm}}{\textbf{SB-P}} & \multicolumn{1}{p{1cm}}{\textbf{Most inf}} & \multicolumn{1}{p{1cm}}{\textbf{Rand}} &  &  & \multicolumn{1}{c}{\textbf{Index}} & \textbf{q} & \textbf{p} & \multicolumn{1}{p{1cm}}{\textbf{Opt Tree}} & \multicolumn{1}{p{1cm}}{\textbf{SB-L}} & \multicolumn{1}{p{1cm}}{\textbf{SB-P}} & \multicolumn{1}{p{1cm}}{\textbf{Most inf}} & \multicolumn{1}{p{1cm}}{\textbf{Rand}} \\ \cline{1-8} \cline{11-18} 
1 & 1 & 2 & 17 & 511 & 511 & 511 & 511 &  &  & 51 & 5 & 5 & 15 & 255 & 255 & 255 & 156 \\
2 & 1 & 2.5 & 17 & 511 & 511 & 511 & 511 &  &  & 52 & 5 & 5.5 & 15 & 255 & 255 & 255 & 129 \\
3 & 1 & 3 & 17 & 511 & 511 & 511 & 511 &  &  & 53 & 5 & 6 & 15 & 255 & 255 & 255 & 255 \\
4 & 1 & 3.5 & 17 & 511 & 511 & 511 & 511 &  &  & 54 & 5 & 6.5 & 15 & 255 & 255 & 255 & 139 \\
5 & 1 & 4 & 17 & 511 & 511 & 511 & 511 &  &  & 55 & 5 & 7 & 15 & 255 & 255 & 255 & 153 \\
6 & 1 & 4.5 & 17 & 511 & 511 & 511 & 511 &  &  & 56 & 6 & 2 & 7 & 15 & 15 & 15 & 15 \\
7 & 1 & 5 & 17 & 511 & 511 & 511 & 511 &  &  & 57 & 6 & 2.5 & 9 & 31 & 31 & 31 & 50 \\
8 & 1 & 5.5 & 17 & 511 & 511 & 511 & 511 &  &  & 58 & 6 & 3 & 11 & 63 & 63 & 63 & 65 \\
9 & 1 & 6 & 17 & 511 & 511 & 511 & 511 &  &  & 59 & 6 & 3.5 & 11 & 63 & 63 & 63 & 96 \\
10 & 1 & 6.5 & 17 & 511 & 511 & 511 & 511 &  &  & 60 & 6 & 4 & 13 & 127 & 127 & 127 & 127 \\
11 & 1 & 7 & 17 & 511 & 511 & 511 & 511 &  &  & 61 & 6 & 4.5 & 13 & 127 & 127 & 127 & 102 \\
12 & 2 & 2 & 15 & 255 & 255 & 255 & 255 &  &  & 62 & 6 & 5 & 13 & 127 & 127 & 127 & 135 \\
13 & 2 & 2.5 & 15 & 255 & 255 & 255 & 113 &  &  & 63 & 6 & 5.5 & 13 & 127 & 127 & 127 & 128 \\
14 & 2 & 3 & 15 & 255 & 255 & 255 & 128 &  &  & 64 & 6 & 6 & 15 & 255 & 255 & 255 & 255 \\
15 & 2 & 3.5 & 15 & 255 & 255 & 255 & 94 &  &  & 65 & 6 & 6.5 & 15 & 255 & 255 & 255 & 129 \\
16 & 2 & 4 & 17 & 511 & 511 & 511 & 511 &  &  & 66 & 6 & 7 & 15 & 255 & 255 & 255 & 158 \\
17 & 2 & 4.5 & 17 & 511 & 511 & 511 & 511 &  &  & 67 & 7 & 2 & 5 & 7 & 7 & 7 & 7 \\
18 & 2 & 5 & 17 & 511 & 511 & 511 & 511 &  &  & 68 & 7 & 2.5 & 7 & 15 & 15 & 15 & 32 \\
19 & 2 & 5.5 & 17 & 511 & 511 & 511 & 511 &  &  & 69 & 7 & 3 & 9 & 31 & 31 & 31 & 51 \\
20 & 2 & 6 & 17 & 511 & 511 & 511 & 511 &  &  & 70 & 7 & 3.5 & 11 & 63 & 63 & 63 & 67 \\
21 & 2 & 6.5 & 17 & 511 & 511 & 511 & 511 &  &  & 71 & 7 & 4 & 11 & 63 & 63 & 63 & 63 \\
22 & 2 & 7 & 17 & 511 & 511 & 511 & 511 &  &  & 72 & 7 & 4.5 & 11 & 63 & 63 & 63 & 84 \\
23 & 3 & 2 & 13 & 127 & 127 & 127 & 127 &  &  & 73 & 7 & 5 & 13 & 127 & 127 & 127 & 109 \\
24 & 3 & 2.5 & 13 & 127 & 127 & 127 & 129 &  &  & 74 & 7 & 5.5 & 13 & 127 & 127 & 127 & 104 \\
25 & 3 & 3 & 15 & 255 & 255 & 255 & 146 &  &  & 75 & 7 & 6 & 13 & 127 & 127 & 127 & 127 \\
26 & 3 & 3.5 & 15 & 255 & 255 & 255 & 120 &  &  & 76 & 7 & 6.5 & 13 & 127 & 127 & 127 & 125 \\
27 & 3 & 4 & 15 & 255 & 255 & 255 & 255 &  &  & 77 & 7 & 7 & 15 & 255 & 255 & 255 & 137 \\
28 & 3 & 4.5 & 15 & 255 & 255 & 255 & 130 &  &  & 78 & 8 & 2 & 3 & 3 & 3 & 3 & 3 \\
29 & 3 & 5 & 15 & 255 & 255 & 255 & 107 &  &  & 79 & 8 & 2.5 & 5 & 7 & 7 & 7 & 16 \\
30 & 3 & 5.5 & 15 & 255 & 255 & 255 & 115 &  &  & 80 & 8 & 3 & 7 & 15 & 15 & 15 & 34 \\
31 & 3 & 6 & 17 & 511 & 511 & 511 & 511 &  &  & 81 & 8 & 3.5 & 9 & 31 & 31 & 31 & 44 \\
32 & 3 & 6.5 & 17 & 511 & 511 & 511 & 511 &  &  & 82 & 8 & 4 & 11 & 63 & 63 & 63 & 63 \\
33 & 3 & 7 & 17 & 511 & 511 & 511 & 511 &  &  & 83 & 8 & 4.5 & 11 & 63 & 63 & 63 & 64 \\
34 & 4 & 2 & 11 & 63 & 63 & 63 & 63 &  &  & 84 & 8 & 5 & 11 & 63 & 63 & 63 & 73 \\
35 & 4 & 2.5 & 11 & 63 & 63 & 63 & 106 &  &  & 85 & 8 & 5.5 & 13 & 127 & 127 & 127 & 113 \\
36 & 4 & 3 & 13 & 127 & 127 & 127 & 129 &  &  & 86 & 8 & 6 & 13 & 127 & 127 & 127 & 127 \\
37 & 4 & 3.5 & 13 & 127 & 127 & 127 & 117 &  &  & 87 & 8 & 6.5 & 13 & 127 & 127 & 127 & 111 \\
38 & 4 & 4 & 15 & 255 & 255 & 255 & 255 &  &  & 88 & 8 & 7 & 13 & 127 & 127 & 127 & 132 \\
39 & 4 & 4.5 & 15 & 255 & 255 & 255 & 149 &  &  & 89 & 9 & 2 & 1 & 1 & 1 & 1 & 1 \\
40 & 4 & 5 & 15 & 255 & 255 & 255 & 138 &  &  & 90 & 9 & 2.5 & 3 & 3 & 3 & 3 & 6 \\
41 & 4 & 5.5 & 15 & 255 & 255 & 255 & 183 &  &  & 91 & 9 & 3 & 7 & 15 & 15 & 15 & 20 \\
42 & 4 & 6 & 15 & 255 & 255 & 255 & 255 &  &  & 92 & 9 & 3.5 & 7 & 15 & 15 & 15 & 31 \\
43 & 4 & 6.5 & 15 & 255 & 255 & 255 & 119 &  &  & 93 & 9 & 4 & 9 & 31 & 31 & 31 & 31 \\
44 & 4 & 7 & 15 & 255 & 255 & 255 & 135 &  &  & 94 & 9 & 4.5 & 11 & 63 & 63 & 63 & 55 \\
45 & 5 & 2 & 9 & 31 & 31 & 31 & 31 &  &  & 95 & 9 & 5 & 11 & 63 & 63 & 63 & 61 \\
46 & 5 & 2.5 & 11 & 63 & 63 & 63 & 75 &  &  & 96 & 9 & 5.5 & 11 & 63 & 63 & 63 & 79 \\
47 & 5 & 3 & 11 & 63 & 63 & 63 & 103 &  &  & 97 & 9 & 6 & 13 & 127 & 127 & 127 & 127 \\
48 & 5 & 3.5 & 13 & 127 & 127 & 127 & 109 & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & 98 & 9 & 6.5 & 13 & 127 & 127 & 127 & 102 \\
49 & 5 & 4 & 13 & 127 & 127 & 127 & 127 & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & 99 & 9 & 7 & 13 & 127 & 127 & 127 & 123 \\
50 & 5 & 4.5 & 13 & 127 & 127 & 127 & 141 & \multicolumn{1}{r}{\textbf{}} & \multicolumn{1}{r}{\textbf{}} & \multicolumn{3}{r}{\textbf{Average}} & \textbf{9} & \textbf{125} & \textbf{125} & \textbf{141} & \textbf{117} \\
 &  &  &  &  &  &  &  & \multicolumn{1}{r}{\textbf{}} & \multicolumn{1}{r}{\textbf{}} & \multicolumn{3}{r}{\textbf{Geo mean}} & \textbf{8} & \textbf{34} & \textbf{34} & \textbf{54} & \textbf{46}
\end{tabular}
\end{adjustwidth}
\end{center}
\end{table}

==> tables/table_vertex_cover_20,25a.tex <==
\begin{table}\small
\begin{center}
\caption{Computational Results for Vertex Cover instances with, $|V|=20,\; p=0.25$}
\begin{adjustwidth}{-0.5in}{-0.5in}
\begin{tabular}{crrrrrrrcrrrrr}
\cline{1-6} \cline{9-14}
\multicolumn{1}{p{1cm}}{\textbf{Index}} & \multicolumn{1}{p{1cm}}{\textbf{Opt Tree}} & \multicolumn{1}{p{1cm}}{\textbf{SB-L}} & \multicolumn{1}{p{1cm}}{\textbf{SB-P}} & \multicolumn{1}{p{1cm}}{\textbf{Most inf}} & \multicolumn{1}{p{1cm}}{\textbf{Rand}} &  &  & \multicolumn{1}{p{1cm}}{\textbf{Index}} & \multicolumn{1}{p{1cm}}{\textbf{Opt Tree}} & \multicolumn{1}{p{1cm}}{\textbf{SB-L}} & \multicolumn{1}{p{1cm}}{\textbf{SB-P}} & \multicolumn{1}{p{1cm}}{\textbf{Most inf}} & \multicolumn{1}{p{1cm}}{\textbf{Rand}} \\ \cline{1-6} \cline{9-14}
1 & 2 & 4 & 2 & 5 & 6 &  &  & 52 & 0 & 0 & 0 & 0 & 0 \\
2 & 3 & 3 & 3 & 7 & 8 &  &  & 53 & 1 & 4 & 4 & 3 & 2 \\
3 & 1 & 1 & 1 & 3 & 3 &  &  & 54 & 2 & 2 & 2 & 4 & 3 \\
4 & 0 & 0 & 0 & 0 & 0 &  &  & 55 & 1 & 2 & 2 & 2 & 2 \\
5 & 0 & 0 & 0 & 0 & 0 &  &  & 56 & 3 & 4 & 3 & 10 & 7 \\
6 & 1 & 1 & 1 & 2 & 2 &  &  & 57 & 0 & 0 & 0 & 0 & 0 \\
7 & 1 & 3 & 3 & 2 & 3 &  &  & 58 & 2 & 2 & 2 & 7 & 4 \\
8 & 2 & 4 & 5 & 6 & 5 &  &  & 59 & 1 & 1 & 1 & 1 & 1 \\
9 & 2 & 2 & 2 & 7 & 3 &  &  & 60 & 3 & 3 & 3 & 7 & 9 \\
10 & 2 & 4 & 2 & 2 & 4 &  &  & 61 & 1 & 2 & 2 & 2 & 2 \\
11 & 4 & 6 & 5 & 14 & 13 &  &  & 62 & 2 & 3 & 3 & 4 & 5 \\
12 & 1 & 1 & 1 & 1 & 1 &  &  & 63 & 1 & 2 & 2 & 3 & 2 \\
13 & 2 & 4 & 3 & 4 & 5 &  &  & 64 & 3 & 4 & 4 & 9 & 8 \\
14 & 1 & 1 & 2 & 3 & 2 &  &  & 65 & 0 & 0 & 0 & 0 & 0 \\
15 & 3 & 3 & 5 & 12 & 8 &  &  & 66 & 1 & 2 & 2 & 3 & 2 \\
16 & 2 & 3 & 3 & 4 & 7 &  &  & 67 & 2 & 4 & 3 & 5 & 4 \\
17 & 3 & 4 & 5 & 11 & 10 &  &  & 68 & 2 & 2 & 2 & 4 & 5 \\
18 & 1 & 2 & 2 & 1 & 1 &  &  & 69 & 0 & 0 & 0 & 0 & 0 \\
19 & 2 & 4 & 4 & 4 & 4 &  &  & 70 & 2 & 3 & 4 & 4 & 4 \\
20 & 1 & 2 & 2 & 2 & 2 &  &  & 71 & 1 & 1 & 1 & 1 & 1 \\
21 & 0 & 0 & 0 & 0 & 0 &  &  & 72 & 1 & 1 & 1 & 2 & 2 \\
22 & 1 & 1 & 2 & 3 & 3 &  &  & 73 & 2 & 2 & 2 & 5 & 5 \\
23 & 0 & 0 & 0 & 0 & 0 &  &  & 74 & 2 & 2 & 2 & 3 & 3 \\
24 & 2 & 3 & 3 & 8 & 5 &  &  & 75 & 1 & 1 & 1 & 2 & 1 \\
25 & 1 & 1 & 1 & 3 & 3 &  &  & 76 & 2 & 2 & 2 & 3 & 3 \\
26 & 0 & 0 & 0 & 0 & 0 &  &  & 77 & 2 & 2 & 2 & 6 & 4 \\
27 & 0 & 0 & 0 & 0 & 0 &  &  & 78 & 3 & 3 & 3 & 6 & 10 \\
28 & 2 & 4 & 3 & 4 & 4 &  &  & 79 & 0 & 0 & 0 & 0 & 0 \\
29 & 2 & 3 & 3 & 10 & 5 &  &  & 80 & 2 & 2 & 2 & 3 & 3 \\
30 & 0 & 0 & 0 & 0 & 0 &  &  & 81 & 2 & 3 & 3 & 10 & 7 \\
31 & 1 & 1 & 1 & 1 & 2 &  &  & 82 & 2 & 2 & 2 & 2 & 3 \\
32 & 2 & 2 & 2 & 2 & 5 &  &  & 83 & 1 & 3 & 1 & 2 & 2 \\
33 & 2 & 2 & 2 & 4 & 5 &  &  & 84 & 1 & 1 & 1 & 4 & 3 \\
34 & 2 & 2 & 2 & 5 & 6 &  &  & 85 & 3 & 4 & 4 & 13 & 12 \\
35 & 0 & 0 & 0 & 0 & 0 &  &  & 86 & 2 & 2 & 2 & 4 & 4 \\
36 & 2 & 3 & 3 & 3 & 3 &  &  & 87 & 0 & 0 & 0 & 0 & 0 \\
37 & 0 & 0 & 0 & 0 & 0 &  &  & 88 & 2 & 4 & 3 & 3 & 7 \\
38 & 3 & 3 & 3 & 6 & 7 &  &  & 89 & 0 & 0 & 0 & 0 & 0 \\
39 & 1 & 1 & 1 & 1 & 1 &  &  & 90 & 0 & 0 & 0 & 0 & 0 \\
40 & 3 & 4 & 4 & 4 & 6 &  &  & 91 & 2 & 4 & 4 & 6 & 4 \\
41 & 2 & 5 & 3 & 3 & 4 &  &  & 92 & 1 & 2 & 2 & 2 & 2 \\
42 & 1 & 2 & 2 & 3 & 3 &  &  & 93 & 0 & 0 & 0 & 0 & 0 \\
43 & 3 & 3 & 4 & 7 & 9 &  &  & 94 & 1 & 1 & 1 & 1 & 1 \\
44 & 3 & 3 & 3 & 5 & 6 &  &  & 95 & 1 & 2 & 2 & 1 & 2 \\
45 & 1 & 2 & 2 & 2 & 3 &  &  & 96 & 2 & 3 & 2 & 3 & 5 \\
46 & 1 & 1 & 1 & 1 & 1 &  &  & 97 & 2 & 3 & 3 & 3 & 4 \\
47 & 0 & 0 & 0 & 0 & 0 &  &  & 98 & 2 & 2 & 2 & 5 & 6 \\
48 & 1 & 1 & 1 & 1 & 2 &  &  & 99 & 0 & 0 & 0 & 0 & 0 \\
49 & 2 & 3 & 3 & 4 & 5 &  &  & 100 & 1 & 1 & 1 & 1 & 1 \\
50 & 1 & 1 & 1 & 1 & 1 & \multicolumn{3}{r}{\textbf{Average}} & \textbf{1} & \textbf{2} & \textbf{2} & \textbf{3} & \textbf{3} \\
51 & 0 & 0 & 0 & 0 & 0 & \multicolumn{3}{r}{\textbf{Geo mean}} & \textbf{2} & \textbf{2} & \textbf{2} & \textbf{3} & \textbf{3}
\end{tabular}
\end{adjustwidth}
\end{center}
\end{table}

==> tables/table_vertex_cover_20,50a.tex <==
\begin{table}\small
\begin{center}
\caption{Computational Results for Vertex Cover instances with $|V|=20, \; p=0.50$}
\begin{adjustwidth}{-0.5in}{-0.5in}
\begin{tabular}{crrrrrrrcrrrrr}
\cline{1-6} \cline{9-14}
\multicolumn{1}{p{1cm}}{\textbf{Index}} & \multicolumn{1}{p{1cm}}{\textbf{Opt Tree}} & \multicolumn{1}{p{1cm}}{\textbf{SB-L}} & \multicolumn{1}{p{1cm}}{\textbf{SB-P}} & \multicolumn{1}{p{1cm}}{\textbf{Most inf}} & \multicolumn{1}{p{1cm}}{\textbf{Rand}} &  &  & \multicolumn{1}{p{1cm}}{\textbf{Index}} & \multicolumn{1}{p{1cm}}{\textbf{Opt Tree}} & \multicolumn{1}{p{1cm}}{\textbf{SB-L}} & \multicolumn{1}{p{1cm}}{\textbf{SB-P}} & \multicolumn{1}{p{1cm}}{\textbf{Most inf}} & \multicolumn{1}{p{1cm}}{\textbf{Rand}} \\ \cline{1-6} \cline{9-14} 
1 & 4 & 7 & 4 & 12 & 10 &  &  & 52 & 4 & 6 & 6 & 8 & 8 \\
2 & 5 & 10 & 9 & 14 & 16 &  &  & 53 & 4 & 7 & 7 & 9 & 12 \\
3 & 3 & 6 & 4 & 10 & 7 &  &  & 54 & 7 & 9 & 8 & 12 & 15 \\
4 & 6 & 9 & 9 & 13 & 12 &  &  & 55 & 5 & 8 & 7 & 13 & 13 \\
5 & 5 & 6 & 6 & 8 & 9 &  &  & 56 & 5 & 8 & 7 & 9 & 10 \\
6 & 3 & 6 & 6 & 6 & 8 &  &  & 57 & 4 & 6 & 6 & 9 & 9 \\
7 & 5 & 8 & 7 & 6 & 10 &  &  & 58 & 5 & 7 & 6 & 14 & 11 \\
8 & 3 & 3 & 3 & 7 & 5 &  &  & 59 & 6 & 9 & 7 & 13 & 11 \\
9 & 6 & 7 & 7 & 21 & 17 &  &  & 60 & 5 & 9 & 10 & 11 & 14 \\
10 & 6 & 10 & 8 & 11 & 13 &  &  & 61 & 2 & 3 & 3 & 5 & 4 \\
11 & 3 & 5 & 3 & 8 & 5 &  &  & 62 & 5 & 6 & 7 & 7 & 10 \\
12 & 4 & 6 & 4 & 11 & 6 &  &  & 63 & 3 & 5 & 5 & 5 & 7 \\
13 & 2 & 4 & 4 & 2 & 4 &  &  & 64 & 5 & 7 & 6 & 11 & 12 \\
14 & 3 & 5 & 4 & 6 & 7 &  &  & 65 & 5 & 7 & 7 & 11 & 9 \\
15 & 7 & 8 & 8 & 10 & 14 &  &  & 66 & 5 & 5 & 7 & 10 & 10 \\
16 & 3 & 7 & 6 & 8 & 8 &  &  & 67 & 5 & 6 & 6 & 8 & 10 \\
17 & 5 & 8 & 8 & 7 & 10 &  &  & 68 & 4 & 7 & 8 & 12 & 9 \\
18 & 5 & 10 & 7 & 16 & 12 &  &  & 69 & 6 & 10 & 8 & 15 & 14 \\
19 & 6 & 10 & 8 & 11 & 14 &  &  & 70 & 6 & 9 & 8 & 12 & 13 \\
20 & 2 & 4 & 4 & 5 & 5 &  &  & 71 & 3 & 6 & 5 & 9 & 8 \\
21 & 5 & 5 & 6 & 9 & 9 &  &  & 72 & 3 & 4 & 4 & 6 & 6 \\
22 & 5 & 8 & 9 & 15 & 15 &  &  & 73 & 3 & 4 & 5 & 6 & 7 \\
23 & 3 & 3 & 7 & 7 & 9 &  &  & 74 & 4 & 5 & 7 & 8 & 13 \\
24 & 5 & 6 & 6 & 15 & 10 &  &  & 75 & 6 & 9 & 9 & 11 & 11 \\
25 & 6 & 9 & 7 & 18 & 13 &  &  & 76 & 4 & 8 & 6 & 10 & 10 \\
26 & 8 & 11 & 11 & 18 & 19 &  &  & 77 & 5 & 8 & 7 & 7 & 10 \\
27 & 5 & 5 & 5 & 9 & 14 &  &  & 78 & 6 & 9 & 9 & 13 & 14 \\
28 & 6 & 7 & 7 & 13 & 10 &  &  & 79 & 7 & 9 & 8 & 12 & 14 \\
29 & 3 & 7 & 5 & 5 & 5 &  &  & 80 & 6 & 8 & 8 & 15 & 14 \\
30 & 5 & 5 & 5 & 9 & 10 &  &  & 81 & 5 & 6 & 6 & 10 & 9 \\
31 & 5 & 5 & 5 & 8 & 9 &  &  & 82 & 5 & 6 & 6 & 9 & 10 \\
32 & 6 & 8 & 8 & 13 & 12 &  &  & 83 & 4 & 5 & 5 & 8 & 12 \\
33 & 3 & 5 & 4 & 7 & 6 &  &  & 84 & 4 & 4 & 5 & 10 & 10 \\
34 & 3 & 5 & 4 & 10 & 6 &  &  & 85 & 5 & 5 & 6 & 9 & 9 \\
35 & 6 & 9 & 9 & 15 & 16 &  &  & 86 & 7 & 10 & 9 & 14 & 16 \\
36 & 3 & 6 & 6 & 4 & 6 &  &  & 87 & 6 & 10 & 8 & 12 & 12 \\
37 & 5 & 6 & 6 & 9 & 11 &  &  & 88 & 5 & 6 & 6 & 12 & 11 \\
38 & 5 & 6 & 5 & 6 & 12 &  &  & 89 & 5 & 7 & 6 & 8 & 9 \\
39 & 4 & 5 & 6 & 7 & 8 &  &  & 90 & 5 & 6 & 6 & 7 & 9 \\
40 & 6 & 7 & 8 & 12 & 10 &  &  & 91 & 4 & 6 & 6 & 5 & 7 \\
41 & 3 & 7 & 7 & 6 & 8 &  &  & 92 & 4 & 5 & 6 & 6 & 9 \\
42 & 4 & 7 & 6 & 7 & 9 &  &  & 93 & 2 & 3 & 3 & 4 & 5 \\
43 & 2 & 5 & 4 & 4 & 6 &  &  & 94 & 5 & 7 & 6 & 10 & 10 \\
44 & 4 & 5 & 5 & 8 & 11 &  &  & 95 & 7 & 9 & 9 & 17 & 15 \\
45 & 5 & 6 & 6 & 8 & 9 &  &  & 96 & 7 & 10 & 8 & 10 & 14 \\
46 & 5 & 5 & 5 & 10 & 9 &  &  & 97 & 5 & 6 & 6 & 11 & 11 \\
47 & 4 & 6 & 5 & 10 & 9 &  &  & 98 & 5 & 7 & 6 & 10 & 12 \\
48 & 3 & 5 & 4 & 6 & 6 &  &  & 99 & 6 & 7 & 8 & 10 & 13 \\
49 & 4 & 5 & 5 & 10 & 8 &  &  & 100 & 7 & 9 & 9 & 21 & 13 \\
50 & 3 & 5 & 5 & 7 & 7 & \multicolumn{3}{r}{\textbf{Average}} & \textbf{5} & \textbf{7} & \textbf{6} & \textbf{10} & \textbf{10} \\
51 & 5 & 7 & 7 & 12 & 9 & \multicolumn{3}{r}{\textbf{Geo mean}} & \textbf{4} & \textbf{6} & \textbf{6} & \textbf{9} & \textbf{10}
\end{tabular}
\end{adjustwidth}
\end{center}
\end{table}
